Code Representation Learning At Scale

Recent studies have shown that code language models at scale demonstrate significant performance gains on downstream tasks, i.e., code generation. However, most of the existing works on code representation learning train models at a hundred million parameter scale using very limited pretraining corpora. In this work, we fuel code representation learning with a vast amount of code data via a two-stage pretraining scheme. We first train the encoders via a mix that leverages both randomness in masking language modeling and the structure aspect of programming language. We then enhance the representations via contrastive learning with hard negative and hard positive constructed in an unsupervised manner. We establish an off-the-shelf encoder model that persistently outperforms the existing models on a wide variety of downstream tasks by large margins. To comprehend the factors contributing to successful code representation learning, we conduct detailed ablations and share our findings on (i) a customized and effective token-level denoising scheme for source code; (ii) the importance of hard negatives and hard positives; (iii) how the proposed bimodal contrastive learning boost the cross-lingual semantic search performance; and (iv) how the pretraining schemes decide the downstream task performance scales with the model size.

==> figures/code2code_search_example.tex <==
\begin{figure*}[t]
\centering
\begin{tabular}{l}

\hline
Query:python how to tell if path passed in is absolute or relative\\
\hline


Relevant Code in Python \\
\hdashline\noalign{\vskip 0.5ex}

\begin{adjustbox}{valign=t,minipage=0.95\textwidth}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomPy}
\begin{lstlisting}
def is_relative_url(url):
    if url.startswith("#"):
        return None
    if url.find("://") > 0 or url.startswith("//"):
        return False
    return True
\end{lstlisting}
\end{tabular}
\end{adjustbox}

\smallskip\\
\hline
Irrelevant Code in Python \\
\hdashline\noalign{\vskip 0.5ex}

\begin{adjustbox}{valign=t,minipage=0.95\textwidth}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomPy}
\begin{lstlisting}
def rel_path(filename):
    return os.path.join(os.getcwd(), os.path.dirname(__file__), filename)
\end{lstlisting}
\end{tabular}
\end{adjustbox}

\smallskip\\ 
\hline
\end{tabular}
\caption{An example of a query and two candidate documents (python functions) from CoSQA text-to-code search task. There are 500 queries in the test split and for every query there is one python function (out of 6,267) that answers it.}
\label{fig:text_to_code_search}
\end{figure*}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{figure*}[t]
\centering
\begin{tabular}{l}

\hline
Query Program in Python\\
\hdashline\noalign{\vskip 0.5ex}

\begin{adjustbox}{valign=t,minipage=0.95\linewidth}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomPy}
\begin{lstlisting}
import math
h,w=map(int, input().split())
if h%3==0 or w%3==0:
    print(0)
else:
    x,y=max(h,w),min(h,w)
    ans=y
    for hi in range(1,h):
        M=max(hi*w,(h-hi)*((w+1)//2),(h-hi)*(w//2))
        m=min(hi*w,(h-hi)*((w+1)//2),(h-hi)*(w//2))
        ans=min(ans,M-m)
    for wi in range(1,w):
        M=max(wi*h,(w-wi)*((h+1)//2),(w-wi)*(h//2))
        m=min(wi*h,(w-wi)*((h+1)//2),(w-wi)*(h//2))        
        ans=min(ans,M-m)
    print(ans)
\end{lstlisting}
\end{tabular}
\end{adjustbox}

\smallskip\\
\hline
Relevant Program in Python \\
\hdashline\noalign{\vskip 0.5ex}

\begin{adjustbox}{valign=t,minipage=0.95\textwidth}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomPy}
\begin{lstlisting}
def solve(H,W):
    p1 = [H//3*W, (H-H//3)*(W//2), (H-H//3)*(W-W//2)]
    p2 = [ceil(H/3)*W, (H-ceil(H/3))*(W//2), (H-ceil(H/3))*(W-W//2)]
    S1 = max(p1)-min(p1)
    S2 = max(p2)-min(p2)
    S3 = 0 if H%3==0 else W
    return min(S1,S2,S3)

from math import ceil
H, W = map(int, input().split())
print(min(solve(H,W), solve(W,H)))
\end{lstlisting}
\end{tabular}
\end{adjustbox}

\smallskip\\
\hline
Relevant Program in Java \\
\hdashline\noalign{\vskip 0.5ex}

\begin{adjustbox}{valign=t,minipage=0.90\textwidth}
\begin{tabular}{l}
\lstset{escapechar=@,style=CustomJava}
\begin{lstlisting}
import java.util.*;
public class Main {
	public static void main(String[] args){
		Scanner sc = new Scanner(System.in);
		long w = sc.nextInt();
		long h = sc.nextInt();
		if(w%3==0 || h%3==0)
			System.out.println(0);
		else
			System.out.println(Math.min(solve(w, h), solve(h, w)));
	}
	static long solve(long w, long h){
		long min = Long.MAX_VALUE;
		for(int i=1;i<h;i++){
			long a = w*i;
			long b, c = 0, 0;
			if(w%2==0){
				b = w/2*(h-i);
				c = b;
				min = Math.min(min, Math.max(a, Math.max(b, c))-Math.min(a, Math.min(b, c)));
			}
			else if((h-i)%2==0){
				b = w*((h-i)/2);
				c = b;
				min = Math.min(min, Math.max(a, Math.max(b, c))-Math.min(a, Math.min(b, c)));
			}
			else{
				b = w*((h-i)/2);
				c = w*((h-i)/2+1);
				min = Math.min(min, Math.max(a, Math.max(b, c))-Math.min(a, Math.min(b, c)));
				b = w/2*(h-i);
				c = (w/2+1)*(h-i);
				min = Math.min(min, Math.max(a, Math.max(b, c))-Math.min(a, Math.min(b, c)));
			}
		}
		return min;
	}
}
\end{lstlisting}
\end{tabular}
\end{adjustbox}

\smallskip\\
\hline
\end{tabular}
\caption{An example of a query and relevant documents in code-to-code search task, where both query and candidates are complete programs that solve a programming problem. In this search task, each program is used as a query and retrieve all programs (from a collection of 11,744/15,594/23,530 programs in Ruby, Python, and Java, respectively) that solve the same problem.}
\label{fig:code_to_code_search}
\end{figure*}

==> sections/1.introduction.tex <==
\section{Introduction}
Large language models (LLMs) pretrained on a massive amount of source code have reshaped the landscape of code generation \citep[][\textit{inter alia}]{codex,palm,starcoder}.
% \citep{codex,codegen,palm,incoder,starcoder}
As an example, the recent release of a 6TB dataset \citep{kocetkov2022stack} comprising source code under permissive licenses 
% across 358 programming languages 
play pivotal roles in promoting the advancement of code language models in present times. Nonetheless, these large corpora are not utilized to develop general-purpose Programming Language (PL) embedding models.  To date, most PL embedding models 
% \citep{codebert,graphcodebert,syncobert,guo-etal-2022-unixcoder,cubert,lachaux2021dobf} 
\citep[][\textit{inter alia}]{codebert,graphcodebert,guo-etal-2022-unixcoder} have no more than 125M parameters and are primarily trained on a few millions of training examples, \eg CodeSearchNet \citep{codesearchnet}.
% with 2.3M samples. 

% As such, the performance is limited, and finetuning with labeled data is still required for many downstream discriminative tasks

% Arguably, ever since CodeBERT \citep{codebert}, 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.98\linewidth]{figures/codesage_plus.png}
    \caption{An overview of the key ingredients of our CodeSage framework for programming language representation learning.}
    \label{fig:codesage_overview}
\end{figure}

% Pretraining objective plays another vital role. As a natural starting point, a rich line of work has adopted the mask language modeling (MLM) objective together with the 80-10-10\footnote{Of the uniformly selected tokens for prediction, 80\% are replaced with the [MASK] token, 10\% are replaced with random tokens, and the remaining stay unchanged} corruption convention originally proposed for text \citep{devlin2018bert} to train PL embeddings. 
% However, we find the 80-10-10 convention sub-optimal for source code. Replacing a subset of tokens with random tokens can drastically disrupt the syntax and semantics of code, which makes the learning too challenging to be effective. 
% However, we find the structured nature of PL makes it more sensitive to the corruption induced by the randomly selected tokens.
% As shown in Section \ref{sec:experiments}, such overdone noise yields sub-optimal performance across different model sizes.
% Further, it's worth noting that the majority of downstream discriminative tasks operate at the sequence level. When aiming to improve representations for immediate use in sequence-level tasks by making them more discriminative, contrastive learning emerges as the preferred option.
% Alone this line, UnixCoder \citep{guo-etal-2022-unixcoder} follows \citet{gao2021simcse} to use \textit{dropout} to form positive pair and set new state-of-the-art results on various discriminative tasks. Nevertheless, \textit{more can be different}.  UnixCoder is trained on CodeSearchNet with 2.3M examples only, whilst we and recent work \citep{dse-zhang} find that using \textit{dropout} as augmentation suffers from supporting long training process, and hence cannot benefit from abundant pretraining data. 


\revision{
Despite the undeniable significance of large-scale data, it's imperative to acknowledge the pivotal role that pretraining objectives play in the training of language models. The prevailing approach for pretraining a bidirectional Transformer encoder to learn representations is through the optimization of a masked language modeling (MLM) objective, as proposed by \citet{devlin2018bert}. The masking scheme in the standard MLM objective follows an 80-10-10 practice.\footnote{Under this scheme, 80\% of the randomly selected tokens for prediction are replaced with the [MASK] token, 10\% are substituted with random tokens, and the remaining tokens remain unchanged.} However, we have noticed that such a masking scheme leads to the development of suboptimal code language models. Since PL data contains a mix of natural language (NL) statements (\ie docstrings, comments) and code snippets, we speculate that replacing masked tokens with a random token could result in replacing an NL token with a PL token, and vice versa (see discussions in Appendix \ref{appendix:subsec_data_discussion}).
% \footnote{In the Stack-Python corpus \citep{kocetkov2022stack}, we found that 31.1\% tokens are identifiers, 26.7\% tokens belong to \{keywords, delimiters, operators\}, and 42.2\% of tokens are literals (among then $\sim$39.2\% tokens are String literals). We discuss these statistics in the Appendix \ref{appendix:subsec_data_discussion}.} 
Consequently, the structure and semantics of the masked source code get disrupted, leading to suboptimal learning of the language model.

While MLM pretraining yields contextual token representations, it's important to highlight that most downstream discriminative tasks primarily function at the sequence level. When the objective is to enhance representations for immediate application in sequence-level tasks by increasing their discriminative power, contrastive learning (CL) emerges as a preferable alternative. Existing works have employed unimodal CL (using Code-Code pairs) \citep{guo-etal-2022-unixcoder, jain-etal-2021-contrastive} or and bimodal CL (using Code-Code and Text-Code pairs) \citep{li-etal-2022-coderetriever} for representation learning. In unimodal CL, a popular choice is to utilize \textit{dropout} augmentation \citet{gao2021simcse} to construct positive code pairs. However, we found that \textit{dropout} augmentation is not training compute-optimal, also indicated by \citet{dse-zhang}. In contrast, bimodal CL becomes an appealing choice, primarily because of the availability of paired code and documentation.
Prior studies utilize functions and their corresponding docstrings to establish the bimodal training pairs. Nonetheless, our preliminary experiments indicated that substantial overlap between docstrings and function signatures simplifies the contrastive learning process (see discussions in Appendix \ref{appendix:subsec_data_discussion}).
% \footnote{Within the Stack-Python corpus, there is a 22.3\% token overlap between tokens in a function's docstring and those in its signature and a 23.1\% overlap between docstring tokens and tokens in the function body.}
}

% To this end, we propose to fuel the encoder-based embedding model with a large amount of training data, i.e., The
% Stack \citep{kocetkov2022stack}, via a two-stage training scheme with customized optimization at each stage. 
To this end, we propose a two-stage training scheme with a large amount of customized pretraining data \citep{kocetkov2022stack}. We depict our proposed CodeSage model in Figure \ref{fig:codesage_overview}. 
We first train the bidirectional encoders via a mix of two objectives complementing each other: identifier deobfuscation (DOBF) and MLM without the 80-10-10 practice. 
Similar to a human programmer, finding meaningful names for obfuscated identifiers necessitates the model to acquire a profound comprehension of code semantics and structure.
% Similar to an experienced programmer, In order to reconstruct the obfuscated identifier names, the model needs to understand the overall structure and the high-level semantics of the code.
% Such conjecture is validated by the better performance of code complexity prediction and NL2Code (natural language-to-code) search attained by DOBF in Table \ref{tab:dobf_vs_random}. 
% Meanwhile, the randomly selected prediction tokens in MLM complement DOBF by encouraging the model to capture other facets of code -- this is important for enriching the training signals, especially for data examples with non-informative identifier names.
Meanwhile, as a more general objective, MLM covers other facets beyond identifiers of code --  this is important for enriching the training signals, especially for data examples with non-informative identifier names.


In the second stage, we leverage the \textit{(text, function)} pairs for bimodal contrastive learning (CL), with text mined from the associated docstring.
% Different from existing work that solely relies on the naturally occurring text and code pairs, we avoid model learning shortcuts by removing function signatures and return statements in code due to the potential lexical overlap with the text as they often both carry the high-level semantics of code. 
\revision{In contrast to existing approaches that primarily rely on naturally occurring text and code pairs, we adopt a strategy to reduce the likelihood of the model learning shortcuts. Our approach involves exclusively utilizing the function body while disregarding the signature and return statements.\footnote{The exclusion of return statements makes the function body resemble general code snippets.}}
We additionally harness CL based on hard negatives identified within the embedding space. We show that such a hard positive and negative construction strategy is simple, yet essential for effective bimodal contrastive learning.

We train three embedding models with different sizes, namely, \oursmall (130M), \ourbase (356M), and \ourlarge (1.3B). We assess the effectiveness of our approach over a wide variety of discriminative tasks, where \oursmall persistently outperforms the previous state-of-the-art models with similar model sizes by a large margin on most tasks.  With increased model size, \ourbase and \ourlarge attains {\color{red} x.y\%} relative improvement on multilingual Code2Code search, {\color{red} x.y\%} relative improvement on nature language to code (NL2Code) search, and {\color{red} x.y\%} on classification tasks. 
To comprehend the factors contributing to successful code representation learning, we meticulously analyze the key components of our framework. Consequently, we present our findings to direct future research endeavors.






==> sections/1.introduction_v1.tex <==
\section{Introduction}

Large language models (LLMs) pretrained on a massive amount of source code have reshaped the landscape of code generation \citep{codex,codegen,palm,incoder,starcoder}. 
% \revision{
The recent release of a 6TB dataset comprising source code under permissive licenses across 358 programming languages is playing a pivotal role in promoting the advancement of novel and improved code language models in present times. Nonetheless, these large corpora are not being fully utilized to develop general purpose code representation learning models, which could have a positive impact on various downstream tasks. For instance, tasks such as code search (including code-to-code or text-to-code scenarios), identification of buggy or vulnerable code \citep{zhou2019devign, tufano2019empirical}, detection of code clones \citep{svajlenko2014towards, wang2020detecting}, and code re-ranking \citep{code-reranker} could all benefit from such models. In a recent study \citep{starcoder}, StarEncoder was pretrained on 400 billion tokens spanning 86 languages. However, this pretraining was conducted for a specific objective. On the other hand, earlier research focusing on general purpose code representation learning \citep{feng-etal-2020-codebert,graphcodebert,guo-etal-2022-unixcoder} employed a dataset containing 2.3M functions in six programming languages \citep{codesearchnet}. 

The realm of natural language processing research extensively studied and showed that the capacity of representation learning models increases alongside the augmentation of model size \citep{liu2020roberta, conneau-etal-2020-unsupervised, ni2021sentence}. Nevertheless, prevailing source code representation models in the literature \citep{codebert,graphcodebert,syncobert,guo-etal-2022-unixcoder} have been limited to 125M parameters. Consequently, whether the extension to larger encoder representation models would yield advantages for downstream tasks remains unexplored.
% }

% \revision{
The goal of this paper is to improve source code understanding by training different sized programming language representation models at a very large scale. We pretrain bidirectional encoders in two stages. At the first stage, we train the encoders via a mix of two objectives: masked language modeling (MLM) \citep{devlin2018bert} and deobfuscation (DOBF) \citep{lachaux2021dobf}. In the second stage, we use a bimodal (natural language and code) contrastive learning (CL) objective that uses an unsupervised hard negatives sampling strategy. The DOBF pre-training objective capitalizes on the structural characteristics of programming languages and pre-trains a model to reconstruct the original form of the obfuscated source code. While in stage one, we used 237M source code files in ten programming languages, in stage two, we use 82M natural language summary and function pairs for contrastive learning.
On a wide variety of downstream tasks, the contrastive learning pretraining elevates the performances with 12\% to 51\% relative improvement over stage-1 pretrained models. 
% In zero-shot setting, our best model \ourlarge outperforms UniXCoder on code to code search by up to 19\% accuracy.
% }

We evaluate the effectiveness of our models on multilingual code search (MCS), natural language to code (NL2Code) and documentation search (NL2Doc) tasks.
Our models outperform previous state of the art by x.y\% average MAP on MCS, x.y\% average MRR on NL2Code and x.y\% on NL2Doc search tasks. We also evaluate our models on code classification tasks, namely, defect prediction, complexity prediction, and runtime error prediction. In all these tasks, our models surpass previous state of the art. Moreover, we showcase the effectiveness our models on code retrieval for augmenting language models for code completion tasks.
To comprehend the factors contributing to successful code representation learning, we meticulously analyze the key components of our framework. Consequently, we present our findings to direct future research endeavors.
% In order to understand what enables effective representation learning, we systematically study the major components of our framework and present the findings that will help driving future works.
% and conclude our findings in Section \ref{sec:ablation}.

% Precisely, we make the following contributions in this work.
% \begin{itemize}
%     \item We leverage a two stage pre-training framework and pretrain 130M, 356M, and 1.3B parameters encoder models for source code representation learning in 10 languages.
%     \item We significantly outperform the previous state-of-the-art on multilingual code search, natural language to code and documentation search, and code classification tasks. We further demonstrate our models' effectiveness for code retrieval to augment language models for code completion tasks.
%     \item \wasi{Dejiao, can you add an statement here to briefly summarize the key points of the analysis section.}
% \end{itemize}












% \revision{
% It has been well studied that language model ability scales with the increasing model size or training data \dejiao{add citations}. To date, most of the PL embedding models \citep{codebert,graphcodebert,syncobert,guo-etal-2022-unixcoder} are no larger than 125M and primarily trained on CodeSearchNet \citep{codesearchnet} with less than three million training examples \dejiao{Wasi, please confirm}, or one or two languages mined from GitHub \citep{cubert,lachaux2021dobf}. As such, the performance is inadequate and finetuning with enough labeled data is still required in both evaluations and real use cases to mitigate the gap.  Further, \textit{more can be different}. The effectiveness of the proposed strategies can vary in presence of large scale training data.  For example, we find variant \textit{dropout}-based contrastive learning that proven to be effective in previous work \citep{guo-etal-2022-unixcoder} \dejiao{add more}, suffer from long training process.  
% }

% \wasi{Wasi will add a radar chart to demonstrate the improvements in all downstream tasks.}



% \dejiao{Wasi, below is a few paragraphs for you to consider for merging.}

% Large language models (LLMs) pretrained on a massive amount of source code have reshaped the landscape of code generation \citep{codex,codegen,palm,incoder,starcoder}. 
% However, the progress on code understanding is comparatively slower, where a strong embedding model excelling in discrimination is still missing for a wide range of downstream tasks, to name a few; various semantic search (\eg code-to-code or text-to-code search), buggy code detection, clone detection, and code re-ranking. 

% It has been well studied that language model ability scales with the increasing model size or training data \dejiao{add citations}. To date, most of the PL embedding models \citep{codebert,graphcodebert,syncobert,guo-etal-2022-unixcoder} are no larger than 125M and primarily trained on CodeSearchNet \citep{codesearchnet} with less than three million training examples \dejiao{Wasi, please confirm}, or one or two languages mined from GitHub \citep{cubert,lachaux2021dobf}. As such, the performance is inadequate and finetuning with enough labeled data is still required in both evaluations and real use cases to mitigate the gap.  Further, \textit{more can be different}. The effectiveness of the proposed strategies can vary in presence of large scale training data.  For example, we find variant \textit{dropout}-based contrastive learning that proven to be effective in previous work \citep{guo-etal-2022-unixcoder} \dejiao{add more}, suffer from long training process.  
% The lack of variety in model size also prevents better understanding of how the performance of different downstream tasks scales with the model size and hence better explorations of effective training recipy towards universal embedding for programming languages.

% Training scheme plays another vital role.  Recently, \citet{starcoder} pretrain an encoder on 400 billion tokens spanning 86 programming languages. However, their pretraining was conducted with the token-level MLM objective together with next sequence prediction, which has been shown less effective in capturing sequence-level semantics \citep{gao2021simcse} \dejiao{add more citations}.   \citet{codet5+}, following \citet{codet5,plbart}, aim to train an unified encoder-decoder architecture to support both code understanding and generation tasks. Despite, they extend the CodeSearchNet data used in \citet{codet5+,plbart} by 50 times via including the GitHub Code \footnote{\url{https://huggingface.co/datasets/codeparrot/github-code}} dataset, we find such models often provide sub-optimal performance on discriminative tasks -- similar findings have been reported in \citet{guo-etal-2022-unixcoder} as well.

% To this end, we fuel the encoder-based embedding model with large amount of training data,  \ie The Stack \dejiao{add citation}, via a two-stage training framework. We first layout a good foundation of contextual embedding via structure-aware Mask Language Modeling (MLM), followed by contrastive learning with customized hard positives and hard negatives to enhance the sequence-level representations. 



% \dejiao{brief summarize the key points of stage-I and stage-II pretraining are missing here.}


% The token-level MLM objective is not enough to well capture the sequence-level semantics in representations \citep{gao2019representation,Wang2020Improving,contextual_word_embeddings,gao2021simcse}. We thereby continue to train the model with a properly designed contrastive learning objective. We focus on two key ingredients -- hard positive and hard negative design. 
% Large batch size allows more effective deep metric learning by comparing each anchor against more in-batch negatives. The phase transition point is present due to false negatives when increasing the batch size. 
% We leverage naturally occurring pairs as positives, \ie docstring, and code, while hard positives are constructed by removing function signatures and return statements to avoid learning shortcuts. As for hard negatives, our goal is to develop a simple yet effective unsupervised hard negatives sampling strategy. Our intuition is that, with large enough training data, the probability of the presence of false negatives within each batch is very small, and hard negatives can thereby be identified according to the distance between the anchor and in-batch negatives in the vector space. 

% We assess the effectiveness of our strategy over a wide range of downstream tasks. We persistently advance the previous state-of-the-art results even if we only train the models with the proposed identifier-aware MLM objective, while our contrastive learning strategy further increases the gap with 12\% to 51\% relative improvement on a wide variety of tasks. In order to understand what enables good representation learning, we systematically study the major components of our framework and conclude our findings in Section \ref{sec:ablation}. 




\begin{figure}
% \vspace{-0.5cm}
\centering
\includegraphics[width=1.0\linewidth]{figures/mlm_dobf.pdf}
\caption{An illustration of the MLM and DOBF objectives. Given an input function, the masked language modeling (MLM) task randomly samples tokens to mask out. In the deobfuscation (DOBF) task, the identifiers are masked out and the model is trained to recover the tokens. \dejiao{Wasi, our hard positive construction, even how we leverage hard negatives have their own novelty. I was thinking we can have an pipeline figure highlighting four crucial components, standard MLM w/o random token \& DOBF for MLM, hard pos\& neg for CL.}
}
\label{fig:mlm_dobf} 
% \vspace{-0.2cm}
\end{figure}


==> tables/main/repobench.tex <==
\begin{table*}[t]
    \begin{center}
    {\normalsize{
        \resizebox{1.0\linewidth}{!} {%
        \def\arraystretch{1.2}%
        % \setlength{\tabcolsep}{5pt}
        \begin{tabular}{c l  c c c c  c c c c c c}
        \toprule
        & \multirow{3}{*}{Model} & \multicolumn{4}{c}{Easy} & \multicolumn{6}{c}{Hard}  \\
        \cmidrule(lr){3-6}
        \cmidrule(lr){7-12}
        & & \multicolumn{2}{c}{XF-F} & \multicolumn{2}{c}{XF-R} & \multicolumn{3}{c}{XF-F} & \multicolumn{3}{c}{XF-R} \\
        \cmidrule(lr){3-4}
        \cmidrule(lr){5-6}
        \cmidrule(lr){7-9}
        \cmidrule(lr){10-12}
        & & acc@1 & acc@3 & acc@1 & acc@3 & acc@1 & acc@3 & acc@5 & acc@1 & acc@3 & acc@5 \\ 
        \midrule
        \parbox[t]{4mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Python}}} &
        CodeBERT & 15.81 & 46.36 & 15.90 & 45.95 & 6.83 & 20.66 & 34.52 & 7.20 & 19.85 & 33.60 \\
        & StarEncoder & 17.57 & 49.83 & 18.57 & 49.05 & 9.78 & 24.96 & 39.16 & 9.75 & 24.47 & 38.27 \\
        & CodeT5+ Embedding & 18.65 & 52.42 & 19.53 & 51.42 & 10.69 & 27.01 & 41.48 & 10.70 & 27.32 & 41.65 \\
        & UnixCoder & 27.02	& 60.14	& 29.23	& 61.95	& 19.86	& 41.4 & 55.74 & 22.5 & 43.12 & 56.93 \\
        \cmidrule(lr){2-12}
        & \oursmall & 29.50 & 62.25 & 31.20 & 63.45 & 21.61 & 43.01 & 57.54 & 25.47 & 46.08 & 58.35 \\
        & \ourbase & 28.79 & 61.69 & 30.03 & 62.60 & 22.66 & 43.54 & 57.7 &	25.00 & 46.40 & 55.98 \\
        & \ourlarge & 29.93	& 62.86 & 32.10 & 64.45 & 23.79 & 45.75 & 59.29 & 26.80 & 47.45 & 60.70 \\
        \midrule
        \parbox[t]{4mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{Java}}} &
        CodeBERT & 16.21 & 48.35 & 15.90 & 47.67 & 7.38 & 22.26 & 36.99 & 6.55 & 20.20 & 34.40 \\
        & StarEncoder & 16.85 & 49.35 & 17.22 & 48.45 & 8.29 & 24.41 & 38.71 & 8.22 & 23.60 & 37.57 \\
        & CodeT5+ Embedding & 17.11 & 49.68 & 20.72 & 53.73 & 8.64 & 25.22 & 40.08 & 12.38 & 29.55 & 44.30 \\
        & UnixCoder & 20.44 & 54.25 & 27.25 & 61.48 & 13.79 & 35.73 & 51.54 & 21.05 & 43.38 & 57.80 \\
        \cmidrule(lr){2-12}
        & \oursmall & 21.22 & 55.95 & 28.32 & 62.72 & 15.36 & 36.69 & 52.66 & 24.05 & 46.73& 60.70 \\
        & \ourbase & 21.36 & 54.97 & 29.62 & 62.68 & 16.05 & 37.91 & 52.76 & 25.02 & 46.38 & 61.12 \\
        & \ourlarge & 21.62 & 56.23 & 30.60 & 64.12 & 17.06 & 39.09 & 54.25 & 25.85 & 47.52 & 61.83 \\
        \bottomrule
        \end{tabular}
        }
    }
    }
    \vspace{-2mm}
    \caption{
    Evaluation results on Repobench-R benchmark.
    }
    \vspace{-2mm}
    \label{tab:repobench}
    \end{center}
\end{table*}
